Mamba-Based Ensemble learning for White Blood Cell Classification

White blood cell (WBC) classification assists in assessing immune health and diagnosing various diseases, yet manual classification is labor-intensive and prone to inconsistencies. Recent advancements in deep learning have shown promise over traditional methods; however, challenges such as data imbalance and the computational demands of modern technologies, such as Transformer-based models which do not scale well with input size, limit their practical application. This paper introduces a novel framework that leverages Mamba models integrated with ensemble learning to improve WBC classification. Mamba models, known for their linear complexity, provide a scalable alternative to Transformer-based approaches, making them suitable for deployment in resource-constrained environments. Additionally, we introduce a new WBC dataset, Chula-WBC-8, for benchmarking. Our approach not only validates the effectiveness of Mamba models in this domain but also demonstrates their potential to significantly enhance classification efficiency without compromising accuracy. The source code can be found at https://github.com/LewisClifton/Mamba-WBC-Classification.

==> figures/misc/mamba_block.tex <==
% Define TikZ Styles
\tikzstyle{trapezium_in} = [trapezium, trapezium stretches=true, trapezium left angle=125, trapezium right angle=125, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!20]
\tikzstyle{trapezium_out} = [trapezium, trapezium stretches=true, trapezium left angle=75, trapezium right angle=75, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!20]
\tikzstyle{process} = [rectangle, minimum width=1.2cm, minimum height=0.8cm, text centered, draw=black, fill=blue!20]
\tikzstyle{activation} = [circle, draw=black, minimum size=1cm, align=center, fill=red!20]
\tikzstyle{residual} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!20]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{dashedbox} = [draw=black, thick, inner sep=10pt, rounded corners]


\begin{figure}[t]
    \centering
    \resizebox{0.6\linewidth}{!}{
        \begin{tikzpicture}[node distance=1.2cm]
    
            % First Linear Layer (Trapezium)
            \node (linear1) [trapezium_in] {Linear Projection};
    
            % Convolution Layer
            \node (conv) [process, above of=linear1] {Causal Conv};
    
            % Activation Sigma
            \node (sigma1) [activation, above of=conv] {$\sigma$};
    
            % SSM Layer
            \node (ssm) [process, above of=sigma1] {Selective SSM};
    
            % X (Multiplication Node)
            \node (sum) [activation, above=0.3cm of ssm] {$\mathbf{\times}$};
    
            % Second Linear Layer (Trapezium)
            \node (linear2) [trapezium_out, above of=sum] {Linear Projection};
    
            % Output Arrow
            \draw [arrow] (linear2.north) -- ++(0,0.75);
    
            % Input Arrow
            \draw[arrow] (0,-1.2) -- (linear1.south);
    
            % Main Flow Arrows
            \draw [arrow] (linear1) -- (conv);
            \draw [arrow] (conv) -- (sigma1);
            \draw [arrow] (sigma1) -- (ssm);
            \draw [arrow] (ssm) -- (sum);
            \draw [arrow] (sum) -- (linear2);
    
            % Residual Connection
            \node (res_linear) [trapezium_in, right=1cm of linear1] {Linear Projection};
            \node (res_sigma) [activation, above=1.34 of res_linear] {$\sigma$};
    
            \draw [arrow] (linear1.east) -- (res_linear.west);
            \draw [arrow] (res_linear) -- (res_sigma);
            \draw [arrow] (res_sigma) |- (sum.east);
    
            % Dashed Box Around Everything
            \node[dashedbox, fit=(linear1) (linear2) (conv) (sigma1) (ssm) (sum) (res_linear) (res_sigma)] {};
    
        \end{tikzpicture}
    }
    \caption{Mamba block}
    \label{fig:vision_mamba_block}
\end{figure}

==> figures/misc/transfer_learning.tex <==
\tikzstyle{data} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=blue!20, align=center]
\tikzstyle{model} = [rectangle, minimum width=1.6cm, minimum height=1cm, text centered, draw=black, fill=green!20, align=center]
\tikzstyle{head} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, draw=black, fill=orange!20, align=center]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{transfer} = [thick,->,>=stealth, dashed]
\tikzstyle{dashedbox} = [draw=black, inner sep=6pt, rounded corners]

\begin{figure}[t]
    \centering
    \resizebox{1.0\linewidth}{!}{
        \begin{tikzpicture}[node distance=0.4cm]
    
            % ImageNet Layer
            \node (imagenet_data) [data] {ImageNet-1K};
            \node (imagenet_model) [model, right of=imagenet_data, xshift=2.2cm] {Feature\\ Extractor};
            \node (imagenet_head) [head, right of=imagenet_model, xshift=2.5cm] {Head\\ (1000 classes)};
            \node (imagenet_pred) [right of=imagenet_head, xshift=2.1cm] {Predictions};
            
            % Label above ImageNet Model
            \node (image_net_label) [below of=imagenet_model, xshift= 1.5cm ,yshift=-6mm] {\footnotesize Pretrained model};

            % Dashed box around Pretrained Model and Head
            \node[dashedbox, fit=(imagenet_model) (imagenet_head)] {};
    
            % BloodMNIST Layer
            \node (bloodmnist_data) [data, below of=imagenet_data, yshift=-2.2cm] {BloodMNIST};
            \node (bloodmnist_model) [model, right of=bloodmnist_data, xshift=2.2cm] {Feature\\ Extractor};
            \node (bloodmnist_head) [head, right of=bloodmnist_model, xshift=2.5cm] {Head\\ (8 classes)};
            \node (bloodmnist_pred) [right of=bloodmnist_head, xshift=2.1cm] {Predictions};

            % Label above BloodMNIST Model
            \node (bloodmnist_label) [below of=bloodmnist_model, xshift= 1.5cm, yshift=-6mm] {\footnotesize Fine-tuned model};

            % Dashed box around Fine-tuned Model and Head for BloodMNIST
            \node[dashedbox, fit=(bloodmnist_model) (bloodmnist_head) ] {};
    
            % Chula Layer
            \node (chula_data) [data, below of=bloodmnist_data, yshift=-2.2cm] {Chula-WBC-8};
            \node (chula_model) [model, right of=chula_data, xshift=2.2cm] {Feature\\ Extractor};
            \node (chula_head) [head, right of=chula_model, xshift=2.5cm] {Head\\ (8 classes)};
            \node (chula_pred) [right of=chula_head, xshift=2.1cm] {Predictions};

            % Label above Chula Model
            \node (chula_label) [below of=chula_model, xshift= 1.5cm ,yshift=-6mm] [align=center]{\footnotesize Further fine-tuned model};

            % Dashed box around Fine-tuned Model and Head for Chu-2 
            \node[dashedbox, fit=(chula_model) (chula_head)] {};
    
            % Arrows (Processing Flow)
            \draw [arrow] (imagenet_data) -- (imagenet_model);
            \draw [arrow] (imagenet_model) -- (imagenet_head);
            \draw [arrow] (imagenet_head) -- (imagenet_pred);
    
            \draw [arrow] (bloodmnist_data) -- (bloodmnist_model);
            \draw [arrow] (bloodmnist_model) -- (bloodmnist_head);
            \draw [arrow] (bloodmnist_head) -- (bloodmnist_pred);
    
            \draw [arrow] (chula_data) -- (chula_model);
            \draw [arrow] (chula_model) -- (chula_head);
            \draw [arrow] (chula_head) -- (chula_pred);
    
            % Knowledge transfer Arrows
            \draw [transfer] (imagenet_model.south) -- node[left, xshift=-0.01cm, yshift=-0.05cm] {\footnotesize Knowledge transfer} (bloodmnist_model.north);
            \draw [transfer] (bloodmnist_model.south) -- node[left, xshift=-0.01cm, yshift=-0.05cm] {\footnotesize Knowledge transfer} (chula_model.north);
    
        \end{tikzpicture}
    }
    \caption{Two-tier transfer learning: A model is pretrained on ImageNet-1K, fine-tuned on BloodMNIST, and further fine-tuned on the Chula-WBC-8 dataset.}
    \label{fig:transfer_learning}
\end{figure}

